Local Whittle estimation of high-dimensional long-run variance and precision matrices

This work develops non-asymptotic theory for estimation of the long-run variance matrix and its inverse, the so-called precision matrix, for high-dimensional time series under general assumptions on the dependence structure including long-range dependence. The estimation involves shrinkage techniques which are thresholding and penalizing versions of the classical multivariate local Whittle estimator. The results ensure consistent estimation in a double asymptotic regime where the number of component time series is allowed to grow with the sample size as long as the true model parameters are sparse. The key technical result is a concentration inequality of the local Whittle estimator for the long-run variance matrix around the true model parameters. In particular, it handles simultaneously the estimation of the memory parameters which enter the underlying model. Novel algorithms for the considered procedures are proposed, and a simulation study and a data application are also provided.

==> LW_largedim_algo.tex <==

\section{Algorithm}
\label{se:algo}

==> LW_largedim_applic.tex <==

\section{Applications}
\label{se:appl}

==> LW_largedim_simul.tex <==

\section{Simulation study}
\label{se:sim}


==> Summary.tex <==

\appendix
\section{Summary}


\begin{proposition} \label{prop:supGhat}
Let $\{X_{n}\}_{n \in \ZZ}$ be a $p$-dimensional stable, Gaussian, centered time series with spectral density $f_{X}$.
Then, there are positive constants $c_{1},c_{2}$ such that 
\begin{equation}
\begin{aligned}
&\Prob \Big( \sup_{D \in \Omega(\varepsilon) } 
| \widehat{G}_{rs}(D) - \E \widehat{G}_{rs}(D) | \geq 
\vertiii{G} \delta \Big)
\\& \hspace{1cm} \leq 
c_{1} \exp(-c_{2} \min \{ 
\delta^2 m^{2-4d_{0,\min}+4\varepsilon} N^{4d_{0,\min}-4\varepsilon-1} , 
\delta m^{1-2d_{0,\max}+2\varepsilon} N^{2 \varepsilon} \}) \label{eq:concreal1},
\end{aligned}
\end{equation}
where
$\Omega(\varepsilon) = \{ D \in \mathcal{M}_{\diag} ~|~ \| D -D_{0} \| \leq \varepsilon \}$.
\end{proposition}


As a corollary of the previous Proposition \eqref{prop:supGhat}, we give the result for having the prior knowledge that the underlying process is multivariate long-range dependent, that is, all memory parameters satisfy $D_{0} \succ 0$.

\begin{proposition} \label{prop:supGhat}
Let $\{X_{n}\}_{n \in \ZZ}$ be a $p$-dimensional stable, Gaussian, centered time series with spectral density $f_{X}$ as in \eqref{eq:f} and $D_{0} \succ 0$.
Then, there are positive constants $c_{1},c_{2}$ such that 
\begin{equation}
\begin{aligned}
&\Prob \Big( \sup_{D \in \Omega(\varepsilon) } 
| \widehat{G}_{rs}(D) - \E \widehat{G}_{rs}(D) | \geq 
\vertiii{G} \delta \Big)
\\& \hspace{1cm} \leq 
c_{1} \exp(-c_{2} \min \{ 
\delta^2 m^{2-4d_{0,\min}+4\varepsilon} N^{4d_{0,\min}-4\varepsilon-1} , 
\delta m^{1-2d_{0,\max}+2\varepsilon} N^{2 \varepsilon} \}) \label{eq:concreal1},
\end{aligned}
\end{equation}
where
$\Omega(\varepsilon) = \{ D \in \mathcal{M}_{\diag} ~|~ \| D -D_{0} \| \leq \varepsilon \}$.
\end{proposition}



















%\textit{(i) $d_{0,r},d_{0,s}>x$}: Note that
%\begin{equation}
%\begin{aligned}
%Q(d_{r},d_{s})
%&=
%\Sigma^{\frac{1}{2}} Q_{m}' \widetilde{T}(d_{r},d_{s})' M \widetilde{T}(d_{r},d_{s}) Q_{m} \Sigma^{\frac{1}{2}} \\
%&=
%\Sigma^{\frac{1}{2}} \mathcal{A}_{N} Q_{m}' \mathcal{A}_{N}^{-1} \widetilde{T}(d_{r},d_{s})' M 
%\widetilde{T}(d_{r},d_{s}) \mathcal{A}_{N}^{-1} Q_{m} \mathcal{A}_{N} \Sigma^{\frac{1}{2}}
%\end{aligned}
%\end{equation}
%with
%\begin{equation}
%\begin{aligned}
%\mathcal{A}_{N}=
%\diag(N^{-d_{0,r}},\dots,N^{-d_{0,r}},N^{-d_{0,s}},\dots,N^{-d_{0,s}}).
%\end{aligned}
%\end{equation}
%\begin{equation}
%\begin{aligned}
%\| B_{m,1} \|
%&=
%\| Q_{m}' \mathcal{A}_{N} \Sigma \mathcal{A}_{N} Q_{m} \|
%\leq
%\| Q_{m} \|^2 \| \mathcal{A}_{N} \Sigma \mathcal{A}_{N} \|
%\\&\leq
%\max\{ \| Q_{1,r,m} \|^{2}, \| Q_{2,s,m} \|^{2} \} ( N^{-2\widetilde{a}_{r}} \| \Sigma_{rr} \| + N^{-2\widetilde{a}_{s}} \| \Sigma_{ss} \|)
%\\&\leq 
%c \vertiii{G} (N^{2d_{0,r}-2d_{0,r}}+N^{2d_{0,s}-2d_{0,s}})
%=
%c \vertiii{G}.
%%\\&=
%%c \vertiii{G} m^{2\max \{d_{0,r},d_{0,s}\}} \lambda_{m}^{-2\max \{d_{0,r},d_{0,s}\}},
%\end{aligned}
%\end{equation}
%\begin{equation}
%\begin{aligned}
%\| B_{m,2} \|_{F}
%=
%\| \Sigma^{\frac{1}{2}} Q_{m}' Q_{m} \Sigma^{\frac{1}{2}} \|_{F}
%=
%\| Q_{m}' \Sigma Q_{m} \|_{F}
%\leq
%\| Q_{m} \|^2 \| \Sigma \|_{F} 
%\leq
%\max\{ \| Q_{1,r,m} \|^{2}, \| Q_{2,s,m} \|^{2} \}  N^{\frac{1}{2}}
%\leq N^{\frac{1}{2}}
%%\\&=
%%c \vertiii{G} m^{2\max \{d_{0,r},d_{0,s}\}} \lambda_{m}^{-2\max \{d_{0,r},d_{0,s}\}},
%\end{aligned}
%\end{equation}
%where we used Lemma \ref{le:ineqFrobSigma}. Furthermore,
%\begin{equation}
%\begin{aligned}
%L_{1,1} 
%= \sup_{(d_{r},d_{s}) \in [a_{r},b_{r}] \times [a_{s},b_{s}]} 
%\| \mathcal{A}_{N}^{-1} \widetilde{T}(d_{r},d_{s})' M \widetilde{T}(d_{r},d_{s}) \mathcal{A}_{N}^{-1} \|
%= N^{d_{0,r}+d_{0,s}} \lambda_{m}^{a_{r}+a_{s}}
%= N^{2 \omega_{1}} m^{d_{0,r}+d_{0,s}-2 \omega_{1}}
%\end{aligned}
%\end{equation}
%and
%\begin{equation}
%\begin{aligned}
%L_{1,2}
%= \sup_{(d_{r},d_{s}) \in [a_{r},b_{r}] \times [a_{s},b_{s}]} 
%\| \widetilde{T}(d_{r},d_{s})' M \widetilde{T}(d_{r},d_{s}) \|
%= \lambda_{m}^{a_{r}+a_{s}}
%\end{aligned}
%\end{equation}
%Then,
%\begin{align}
%&
%\Prob \Big( \sup_{(d_{r},d_{s}) \in 
%[a_{r},b_{r}] \times [a_{s},b_{s}]} | \mathcal{E}' Q(d_{r},d_{s}) \mathcal{E}  - 
%\E (\mathcal{E}' Q(d_{r},d_{s}) \mathcal{E} ) | \geq \frac{2 \pi m}{4} \vertiii{G} \nu \Big) 
%\\&\leq
%c \exp\Bigg( - \frac{1}{c} \min 
%\Bigg\{ 
%\frac{ m \vertiii{G} \nu }{ \| B_{m,1} \| L_{1,1} },
%\frac{ (m \vertiii{G} \nu)^2 }{ \| B_{m,2} \|^2_{F} L_{1,2}^{2} }
%\Bigg\} \Bigg) \label{eq:applyDicker1}
%\\ &\leq
%c \exp(-c \min \{ 
%\nu m^{1-d_{0,r}-d_{0,s}+2 \omega_{1}} N^{-2 \omega_{1}},
%\nu^{2} m^{2} N^{-1} \lambda_{m}^{-2a_{r}-2a_{s}}
%\}) 
%\\ &\leq
%c \exp(-c \min \{ 
%\nu m^{1-2\Delta_{2}} N^{-2 \omega_{1}},
%\nu^{2} m^{2} N^{-1} \lambda_{m}^{-2a_{r}-2a_{s}}
%\}) 
%\end{align}
%\vspace{3cm}\\
%\textit{(ii) $0 \leq d_{0,r},d_{0,s}<x$} \\
%Note that
%\begin{equation}
%\begin{aligned}
%Q(d_{r},d_{s})
%&=
%\Sigma^{\frac{1}{2}} Q_{m}' \widetilde{T}(d_{r},d_{s})' M \widetilde{T}(d_{r},d_{s}) Q_{m} \Sigma^{\frac{1}{2}} \\
%&=
%\Sigma^{\frac{1}{2}} \mathcal{A}_{N} Q_{m}' \mathcal{A}_{N}^{-1} \widetilde{T}(d_{r},d_{s})' M 
%\widetilde{T}(d_{r},d_{s}) \mathcal{A}_{N}^{-1} Q_{m} \mathcal{A}_{N} \Sigma^{\frac{1}{2}}
%\end{aligned}
%\end{equation}
%with
%\begin{equation}
%\begin{aligned}
%\mathcal{A}_{N}=
%\diag(N^{-d_{0,r}},\dots,N^{-d_{0,r}},N^{-d_{0,s}},\dots,N^{-d_{0,s}}).
%\end{aligned}
%\end{equation}
%\begin{equation}
%\begin{aligned}
%\| B_{m,1} \|
%&=
%\| Q_{m}' \mathcal{A}_{N} \Sigma \mathcal{A}_{N} Q_{m} \|
%\leq
%\| Q_{m} \|^2 \| \mathcal{A}_{N} \Sigma \mathcal{A}_{N} \|
%\\&\leq
%\max\{ \| Q_{1,r,m} \|^{2}, \| Q_{2,s,m} \|^{2} \} ( N^{-2\widetilde{a}_{r}} \| \Sigma_{rr} \| + N^{-2\widetilde{a}_{s}} \| \Sigma_{ss} \|)
%\\&\leq 
%c \vertiii{G} 
%\end{aligned}
%\end{equation}
%Furthermore,
%\begin{equation}
%\begin{aligned}
%L_{1,2} 
%= \sup_{(d_{r},d_{s}) \in [a_{r},b_{r}] \times [a_{s},b_{s}]}
% \| \mathcal{A}_{N}^{-1} \widetilde{T}(d_{r},d_{s})' M \widetilde{T}(d_{r},d_{s}) \mathcal{A}_{N}^{-1} \|
%= N^{d_{0,r}+d_{0,s}} \lambda_{m}^{a_{r}+a_{s}}
%=N^{2\omega_{1}}m^{d_{0,r}+d_{0,s}-2 \omega_{1}}
%\end{aligned}
%\end{equation}
%and
%\begin{equation}
%\begin{aligned}
%L_{2,2}
%&= \sup_{(d_{r},d_{s}) \in [a_{r},b_{r}] \times [a_{s},b_{s}]}
% \| \mathcal{A}_{N}^{-1} \widetilde{T}(d_{r},d_{s})' M \widetilde{T}(d_{r},d_{s}) \mathcal{A}_{N}^{-1} \|_{F} \\
%&= N^{\widetilde{a}_{r}+\widetilde{a}_{s}} \Big( \sum_{j=1}^{m} \lambda_{j}^{2a_{r}+2a_{s}} \Big)^{\frac{1}{2}}
%\leq 
%N^{2 \omega} (m^{1+2a_{r}+2a_{s}})^{\frac{1}{2}}.
%\end{aligned}
%\end{equation}
%Then,
%\begin{align}
%&
%\Prob \Big( \sup_{(d_{r},d_{s}) \in 
%[a_{r},b_{r}] \times [a_{s},b_{s}]} | \mathcal{E}' Q(d_{r},d_{s}) \mathcal{E}  - 
%\E (\mathcal{E}' Q(d_{r},d_{s}) \mathcal{E} ) | \geq \frac{2 \pi m}{4} \vertiii{G} \nu \Big) 
%\\&\leq
%c \exp\Bigg( - \frac{1}{c} \min 
%\Bigg\{ 
%\frac{ m \vertiii{G} \nu }{ \| B_{m,1} \| L_{1,1} },
%\frac{ (m \vertiii{G} \nu)^2 }{ \| B_{m,2} \|^2_{F} L_{1,2}^{2} }
%\Bigg\} \Bigg) \label{eq:applyDicker1}
%\\ &\leq
%c \exp(-c \min \{ 
%\nu m N^{-d_{0,r}-d_{0,s}} \lambda_{m}^{-a_{r}-a_{s}},
%\nu^{2} m^{2} (N^{4 \omega} m^{1+2a_{r}+2a_{s}})^{-1}
%\}) 
%\end{align}
%\vspace{3cm}\\
%\textit{(iii) $d_{0,r},d_{0,s} < 0$} \\
%\begin{equation}
%\begin{aligned}
%\| B_{m,1} \|
%&=
%\| \Sigma^{\frac{1}{2}} Q_{m}' Q_{m} \Sigma^{\frac{1}{2}} \|
%=
%\| Q_{m}' \Sigma Q_{m} \|
%\leq
%\| Q_{m} \|^2 \| \Sigma \|
%\\&\leq
%\max\{ \| Q_{1,r,m} \|^{2}, \| Q_{2,s,m} \|^{2} \} (\| \Sigma_{rr} \| + \| \Sigma_{ss} \|)
%\\&\leq 
%c \vertiii{G}.
%%\\&=
%%c \vertiii{G} m^{2\max \{d_{0,r},d_{0,s}\}} \lambda_{m}^{-2\max \{d_{0,r},d_{0,s}\}},
%\end{aligned}
%\end{equation}
%Furthermore,
%\begin{equation}
%\begin{aligned}
%L_{1,1} 
%= \sup \| \widetilde{T}(d_{r},d_{s})' M \widetilde{T}(d_{r},d_{s}) \|
%= \lambda_{1}^{a_{r}+a_{s}}
%\end{aligned}
%\end{equation}
%and
%\begin{equation}
%\begin{aligned}
%L_{2,1}
%= \sup \| \widetilde{T}(d_{r},d_{s})' M \widetilde{T}(d_{r},d_{s}) \|_{F}
%= \Big( \sum_{j=1}^{m}\lambda_{j}^{2a_{r}+2a_{s}} \Big)^{\frac{1}{2}}
%\end{aligned}
%\end{equation}
%Then,
%\begin{align}
%&
%\Prob \Big( \sup_{(d_{r},d_{s}) \in 
%[a_{r},b_{r}] \times [a_{s},b_{s}]} | \mathcal{E}' Q(d_{r},d_{s}) \mathcal{E}  - 
%\E (\mathcal{E}' Q(d_{r},d_{s}) \mathcal{E} ) | \geq \frac{2 \pi m}{4} \vertiii{G} \nu \Big) 
%\\&\leq
%c \exp\Bigg( - \frac{1}{c} \min 
%\Bigg\{ 
%\frac{ m \vertiii{G} \nu }{ \| B_{m,1} \| L_{1,1} },
%\frac{ (m \vertiii{G} \nu)^2 }{ \| B_{m,1} \|^2 L_{2,1}^{2} }
%\Bigg\} \Bigg) \label{eq:applyDicker1}
%\\ &\leq
%c \exp(-c \min \{ 
%\nu m \lambda_{1}^{-a_{r}-a_{s}},
%\nu^{2} m^{2} \Big(\sum_{j=1}^{m}\lambda_{j}^{2a_{r}+2a_{s}}\Big)^{-1}
%\}) 
%\\ &\leq
%c \exp(-c \min \{ 
%\nu m N^{2 \Delta_{1}} ,
%\nu^{2} m^{2} \Big( \sum_{j=1}^{m}\lambda_{j}^{4 \Delta_{1} } \Big)^{-1}
%\}) 
%\end{align}
%\vspace{3cm}\\
%\textit{(iv) $d_{0,r}>x, 0 \leq d_{0,s}<x$}: Note that
%\begin{equation}
%\begin{aligned}
%Q(d_{r},d_{s})
%&=
%\Sigma^{\frac{1}{2}} Q_{m}' \widetilde{T}(d_{r},d_{s})' M \widetilde{T}(d_{r},d_{s}) Q_{m} \Sigma^{\frac{1}{2}} \\
%&=
%\Sigma^{\frac{1}{2}} \mathcal{A}_{N} Q_{m}' \mathcal{A}_{N}^{-1} \widetilde{T}(d_{r},d_{s})' M 
%\widetilde{T}(d_{r},d_{s}) \mathcal{A}_{N}^{-1} Q_{m} \mathcal{A}_{N} \Sigma^{\frac{1}{2}}
%\end{aligned}
%\end{equation}
%with
%\begin{equation}
%\begin{aligned}
%\mathcal{A}_{N}=
%\diag(N^{-d_{0,r}},\dots,N^{-d_{0,r}},N^{-d_{0,s}},\dots,N^{-d_{0,s}}).
%\end{aligned}
%\end{equation}
%
%\begin{equation}
%\begin{aligned}
%\| B_{m,1} \|
%&=
%\| \Sigma^{\frac{1}{2}} \mathcal{A}_{N} Q_{m}' Q_{m} \mathcal{A}_{N} \Sigma^{\frac{1}{2}} \|
%=
%\| Q_{m}' \mathcal{A}_{N} \Sigma \mathcal{A}_{N} Q_{m} \|
%\leq
%\| Q_{m} \|^2 \| \mathcal{A}_{N} \Sigma \mathcal{A}_{N} \|
%\\&\leq
%\max\{ \| Q_{1,r,m} \|^{2}, \| Q_{2,s,m} \|^{2} \} ( N^{-2 d_{0,r}} \| \Sigma_{rr} \| + N^{-2d_{0,s}} \| \Sigma_{ss} \|)
%\\&\leq 
%c \vertiii{G}.
%\end{aligned}
%\end{equation}
%\begin{equation}
%\begin{aligned}
%\| B_{m,2} \|_{F}
%=
%\| \Sigma^{\frac{1}{2}} Q_{m}' Q_{m} \Sigma^{\frac{1}{2}} \|_{F}
%=
%\| Q_{m}' \Sigma Q_{m} \|_{F}
%\leq
%\| Q_{m} \|^2 \| \Sigma \|_{F} 
%\leq
%\max\{ \| Q_{1,r,m} \|^{2}, \| Q_{2,s,m} \|^{2} \}  N^{\frac{1}{2}}
%\leq N^{\frac{1}{2}}
%%\\&=
%%c \vertiii{G} m^{2\max \{d_{0,r},d_{0,s}\}} \lambda_{m}^{-2\max \{d_{0,r},d_{0,s}\}},
%\end{aligned}
%\end{equation}
%Furthermore,
%\begin{equation}
%\begin{aligned}
%L_{1,1} 
%= \sup_{(d_{r},d_{s}) \in [a_{r},b_{r}] \times [a_{s},b_{s}]}  
%\| \mathcal{A}_{N}^{-1} \widetilde{T}(d_{r},d_{s})' M \widetilde{T}(d_{r},d_{s}) \mathcal{A}_{N}^{-1} \|
%= N^{d_{0,r}+d_{0,s}} \lambda_{m}^{a_{r}+a_{s}}
%\end{aligned}
%\end{equation}
%\begin{equation}
%\begin{aligned}
%L_{1,2} 
%= \sup_{(d_{r},d_{s}) \in [a_{r},b_{r}] \times [a_{s},b_{s}]}  
%\| \widetilde{T}(d_{r},d_{s})' M \widetilde{T}(d_{r},d_{s}) \|
%= \lambda_{m}^{a_{r}+a_{s}}
%\end{aligned}
%\end{equation}
%Then,
%\begin{align}
%&
%\Prob \Big( \sup_{(d_{r},d_{s}) \in [a_{r},b_{r}] \times [a_{s},b_{s}]} 
%| \mathcal{E}' Q(d_{r},d_{s}) \mathcal{E}  - 
%\E (\mathcal{E}' Q(d_{r},d_{s}) \mathcal{E} ) | \geq \frac{2 \pi m}{4} \vertiii{G} \nu \Big) 
%\\&\leq
%c \exp\Bigg( - \frac{1}{c} \min 
%\Bigg\{ 
%\frac{ m \vertiii{G} \nu }{ \| B_{m,1} \| L_{1,1} },
%\frac{ (m \vertiii{G} \nu)^2 }{ \| B_{m,2} \|^2_{F} L_{1,2}^{2} }
%\Bigg\} \Bigg) \label{eq:applyDicker1}
%\\ &\leq
%c \exp(-c \min \{ 
%\nu m N^{-d_{0,r}-d_{0,s}} \lambda_{m}^{-a_{r}-a_{s}},
%\nu^{2} m^{2} N^{-1} \lambda_{m}^{-2a_{r}-2a_{s}}
%\}) 
%\\ &=
%c \exp(-c \min \{ 
%\nu m^{1-d_{0,r}-d_{0,s}} \lambda_{m}^{2\omega_{1}},
%\nu^{2} m^{2} N^{-1} \lambda_{m}^{-2a_{r}-2a_{s}}
%\}) 
%\end{align}
%\vspace{3cm}\\
%\textit{(v) $d_{0,r}>x, d_{0,s}<0$} \\
%Note that
%\begin{equation}
%\begin{aligned}
%Q(d_{r},d_{s})
%&=
%\Sigma^{\frac{1}{2}} Q_{m}' \widetilde{T}(d_{r},d_{s})' M \widetilde{T}(d_{r},d_{s}) Q_{m} \Sigma^{\frac{1}{2}} \\
%&=
%\Sigma^{\frac{1}{2}} \mathcal{A}_{N} Q_{m}' \mathcal{A}_{N}^{-1} \widetilde{T}(d_{r},d_{s})' M 
%\widetilde{T}(d_{r},d_{s}) \mathcal{A}_{N}^{-1} Q_{m} \mathcal{A}_{N} \Sigma^{\frac{1}{2}}
%\end{aligned}
%\end{equation}
%with
%\begin{equation}
%\begin{aligned}
%\mathcal{A}_{N}=
%\diag(N^{-d_{0,r}},\dots,N^{-d_{0,r}},1,\dots,1).
%\end{aligned}
%\end{equation}
%\begin{equation}
%\begin{aligned}
%\| B_{m,1} \|
%&=
%\| \Sigma^{\frac{1}{2}} Q_{m}' Q_{m} \Sigma^{\frac{1}{2}} \|
%=
%\| Q_{m}' \mathcal{A}_{N} \Sigma \mathcal{A}_{N} Q_{m} \|
%\leq
%\| Q_{m} \|^2 \| \mathcal{A}_{N} \Sigma \mathcal{A}_{N} \|
%\\&\leq
%\max\{ \| Q_{1,r,m} \|^{2}, \| Q_{2,s,m} \|^{2} \} ( N^{-2\widetilde{a}_{r}} \| \Sigma_{rr} \| + \| \Sigma_{ss} \|)
%\\&\leq 
%c \vertiii{G} (N^{2d_{0,r}-2d_{0,r}}+1)
%=
%c \vertiii{G}
%\end{aligned}
%\end{equation}
%Furthermore,
%\begin{equation}
%\begin{aligned}
%L_{1,1} 
%= \sup \| \mathcal{A}_{N}^{-1} \widetilde{T}(d_{r},d_{s})' M \widetilde{T}(d_{r},d_{s}) \mathcal{A}_{N}^{-1} \|
%= N^{d_{0,r}} \max\{ \lambda_{1}^{a_{r}+a_{s}} , \lambda_{m}^{a_{r}+a_{s}} \}
%\end{aligned}
%\end{equation}
%and
%\begin{equation}
%\begin{aligned}
%L_{2,1}
%= \sup \| \mathcal{A}_{N}^{-1} \widetilde{T}(d_{r},d_{s})' M \widetilde{T}(d_{r},d_{s}) \mathcal{A}_{N}^{-1} \|_{F}
%= N^{\widetilde{a}_{r}} \Big( \sum_{j=1}^{m}\lambda_{j}^{2a_{r}+2a_{s}} \Big)^{\frac{1}{2}}
%\end{aligned}
%\end{equation}
%Then,
%\begin{align}
%&
%\Prob \Big( \sup_{(d_{r},d_{s}) \in 
%[a_{r},b_{r}] \times [a_{s},b_{s}]} | \mathcal{E}' Q(d_{r},d_{s}) \mathcal{E}  - 
%\E (\mathcal{E}' Q(d_{r},d_{s}) \mathcal{E} ) | \geq \frac{2 \pi m}{4} \vertiii{G} \nu \Big) 
%\\&\leq
%c \exp\Bigg( - \frac{1}{c} \min 
%\Bigg\{ 
%\frac{ m \vertiii{G} \nu }{ \| B_{m,1} \| L_{1,1} },
%\frac{ (m \vertiii{G} \nu)^2 }{ \| B_{m,1} \|^2 L_{2,1}^{2} }
%\Bigg\} \Bigg) \label{eq:applyDicker1}
%\\ &\leq
%c \exp(-c \min \{ 
%\nu m \lambda_{1}^{-a_{r}-a_{s}},
%\nu^{2} m^{2} \Big(\sum_{j=1}^{m}\lambda_{j}^{2a_{r}+2a_{s}}\Big)^{-1}
%\}) 
%\end{align}
%\vspace{3cm}\\
%\textit{(vi) $0 \leq d_{0,r}<x, d_{0,s}<0$} \\
%Note that
%\begin{equation}
%\begin{aligned}
%Q(d_{r},d_{s})
%&=
%\Sigma^{\frac{1}{2}} Q_{m}' \widetilde{T}(d_{r},d_{s})' M \widetilde{T}(d_{r},d_{s}) Q_{m} \Sigma^{\frac{1}{2}} \\
%&=
%\Sigma^{\frac{1}{2}} \mathcal{A}_{N} Q_{m}' \mathcal{A}_{N}^{-1} \widetilde{T}(d_{r},d_{s})' M 
%\widetilde{T}(d_{r},d_{s}) \mathcal{A}_{N}^{-1} Q_{m} \mathcal{A}_{N} \Sigma^{\frac{1}{2}}
%\end{aligned}
%\end{equation}
%with
%\begin{equation}
%\begin{aligned}
%\mathcal{A}_{N}=
%\diag(N^{-d_{0,r}},\dots,N^{-d_{0,r}},1,\dots,1).
%\end{aligned}
%\end{equation}
%\begin{equation}
%\begin{aligned}
%\| B_{m,1} \|
%&=
%\| \Sigma^{\frac{1}{2}} Q_{m}' Q_{m} \Sigma^{\frac{1}{2}} \|
%=
%\| Q_{m}' \Sigma Q_{m} \|
%\leq
%\| Q_{m} \|^2 \| \Sigma \|
%\\&\leq
%\max\{ \| Q_{1,r,m} \|, \| Q_{2,s,m} \| \} ( N^{-2\widetilde{a}_{r}} \| \Sigma_{rr} \| + \| \Sigma_{ss} \|)
%\\&\leq 
%c \vertiii{G} (N^{2d_{0,r}-2\widetilde{a}_{r}}+1)
%=
%c \vertiii{G}.
%%\\&=
%%c \vertiii{G} m^{2\max \{d_{0,r},d_{0,s}\}} \lambda_{m}^{-2\max \{d_{0,r},d_{0,s}\}},
%\end{aligned}
%\end{equation}
%Furthermore,
%\begin{equation}
%\begin{aligned}
%L_{1,1} 
%= \sup \| \mathcal{A}_{N}^{-1} \widetilde{T}(d_{r},d_{s})' M \widetilde{T}(d_{r},d_{s}) \mathcal{A}_{N}^{-1} \|
%= N^{d_{0,r}} \lambda_{1}^{a_{r}+a_{s}}
%\end{aligned}
%\end{equation}
%and
%\begin{equation}
%\begin{aligned}
%L_{2,1}
%= \sup \| \widetilde{T}(d_{r},d_{s})' M \widetilde{T}(d_{r},d_{s}) \|_{F}
%= \Big( \sum_{j=1}^{m}\lambda_{j}^{2a_{r}+2a_{s}} \Big)^{\frac{1}{2}}
%\end{aligned}
%\end{equation}
%Then,
%\begin{align}
%&
%\Prob \Big( \sup_{(d_{r},d_{s}) \in 
%[a_{r},b_{r}] \times [a_{s},b_{s}]} | \mathcal{E}' Q(d_{r},d_{s}) \mathcal{E}  - 
%\E (\mathcal{E}' Q(d_{r},d_{s}) \mathcal{E} ) | \geq \frac{2 \pi m}{4} \vertiii{G} \nu \Big) 
%\\&\leq
%c \exp\Bigg( - \frac{1}{c} \min 
%\Bigg\{ 
%\frac{ m \vertiii{G} \nu }{ \| B_{m,1} \| L_{1,1} },
%\frac{ (m \vertiii{G} \nu)^2 }{ \| B_{m,1} \|^2 L_{2,1}^{2} }
%\Bigg\} \Bigg) \label{eq:applyDicker1}
%\\ &\leq
%c \exp(-c \min \{ 
%\nu m \lambda_{1}^{-a_{r}-a_{s}},
%\nu^{2} m^{2} \Big(\sum_{j=1}^{m}\lambda_{j}^{2a_{r}+2a_{s}}\Big)^{-1}
%\}) 
%\end{align}





==> natbib/README <==
                                 What is NATBIB?
                                 
It is a LaTeX (2e, with some support for 2.09) package to act as generalized
interface for standard and non-standard bibliographic style files (BibTeX).

It is intended primarily to produce author-year style citations from a variety
of non-standard .bst outputs; it therefore replaces the special and individual
packages that go along with such .bst files:
   apalike.sty    for    apalike.bst et al.
   newapa.sty            newapa.bst, 
   chicago.sty           chicago.bst, named.bst et al.
   harvard.sty           agsm.bst, dcu.bst, kluwer.bst et al.
   astron.sty            astron.bst, apa.bst, humanbio.bst, et al.
   authordate<n>.sty     authordate<n>.bst, aaai-named.bst
   
The above .bst files may also be used with natbib to produce author-year or 
numerical citations, so that switching from author-year to numerical is only 
a matter of selecting an option. 

The standard .bst files (plain et al) and other numerical citation .bst files
are also understood, but they can produce only numerical citations.
Replacement .bst files
   plainnat.bst
   abbrvnat.bst
   unsrtnat.bst
are provided to produce the same formatting of the reference list as the
standard equivalent, but allowing both author-year and numerical citations.

See my parallel custom-bib system for generating customized bst files.

For installation instructions and more details, see README.vxx.

Patrick W. Daly
Max-Planck-Institut f\"ur Sonnensystemforschung
D-37191 Katlenburg-Lindau, Germany
E-mail: daly@mps.mpg.de

